Between Randomness and Arbitrariness: Some Lessons for Reliable Machine Learning at Scale

To develop rigorous knowledge about ML models -- and the systems in which they are embedded -- we need reliable measurements. But reliable measurement is fundamentally challenging, and touches on issues of reproducibility, scalability, uncertainty quantification, epistemology, and more. This dissertation addresses criteria needed to take reliability seriously: both criteria for designing meaningful metrics, and for methodologies that ensure that we can dependably and efficiently measure these metrics at scale and in practice. In doing so, this dissertation articulates a research vision for a new field of scholarship at the intersection of machine learning, law, and policy. Within this frame, we cover topics that fit under three different themes: (1) quantifying and mitigating sources of arbitrariness in ML, (2) taming randomness in uncertainty estimation and optimization algorithms, in order to achieve scalability without sacrificing reliability, and (3) providing methods for evaluating generative-AI systems, with specific focuses on quantifying memorization in language models and training latent diffusion models on open-licensed data. By making contributions in these three themes, this dissertation serves as an empirical proof by example that research on reliable measurement for machine learning is intimately and inescapably bound up with research in law and policy. These different disciplines pose similar research questions about reliable measurement in machine learning. They are, in fact, two complementary sides of the same research vision, which, broadly construed, aims to construct machine-learning systems that cohere with broader societal values.

==> section/10-intro/12-accountability/9999-accountability-coda.tex <==
\section{Coda}\label{sec:acc:coda}

\todo{everything we've said is harder -- relational, not just moral; emphasis on this; emphasis on responsibility; emphasis on robustness aspects; many hands (does not have to be this way, is a functional of how stuff happens in practice; not a condition of software, but how systems built and deployed)}

\todo{not just about legal issues; also moral, notion of of accountable actor and forum}

\todo{many hands section; 4 problems for software (at the top); not just licensed software, but also procurement of enterprise systems}

\todo{pipeline, now supply chain; really an ecosystem; in our formulation, collapsed a bunch of things into problem formulation, where now a lot more complicated; data collection / scraping from web its own whole thing; might then get used by someone else for a task/ thing to learn; evaluation also not about one metric, not super well defined in current day; also loops and iterations (got this right), but also involves a lot of different actors at different organization (more complex now); deployment also not always by same actors now}
\todo{freely available software for download. got the part about pre-trained models; point about investment and reuse. also lmao BERT as the example; recursive nature... but not just this --- missed the boat here. now also about systems, so also APIs and communicating components}

\todo{``bugs'' --- all kinds of ``bad'' new behaviors, all kinds of new scenarios where old ascription to bugs gets deployed (cite paper with James); all kinds of other places (systems-level stuff) where could deal with things that we have trouble controlling at the model level}

\todo{bugs confusing -- turned on their head in ML, when actually features. see this with memorization vs. generalization. point to James paper; over-emphasis on accuracy (discriminative); models (as opposed to systems), even though the paper makes the point about systems}

\todo{lack moral agency; but also now claims of AGI, agentic behaviors; do not ascribe to this, even if ``pass the Turing test.'' Just makes it even messier; anthropomorphization more of thing also with things like chatbots, agentic behaviors; blame ChatGPT for hallucinating, memorizing, regurgitating}

\todo{nondeterminism even more complicated than presented here; cslaw paper; arbitrariness vs. randomness --- aaai, plsc. and even more present with generative AI systems, very different outputs for the same inputs, flips between yes and no on question answering, etc. and being used in high-stakes scenarios. BLaming chatgpt / scape-goating the system; having poor evals to even capture this behavior in the first place}

\todo{ownership without liability: 1) strengthening property rights and 2) avoiding liability.; farcical how much this is a thing right now, terms of service over how to use outputs, but complete disregard for inputs. fair use defenses; LAION an incredible example of this, wrt URLs as a way to sidestep; and then the ultimate presence of CSAM.}

\todo{trade secrets --- worse, with respect to training data; problems for procurement; scape-goating the user (wrt regurgitation and memorization); only possible if the model has memorized something); nailed point on data and misuse; in fact, a twist on this again; relies on past issues of not doing accountability right, e.g., with licenses and early internet; leveraged this via scraping, diffused responsibility this way}

==> section/20-arbitrary/23-nondeterminism/999-nondeterminism-coda.tex <==
\section{Coda} \label{sec:nondeterminism:coda}

As noted at the start of this chapter, the work presented here represents early thoughts on the relevance of machine-learning-based arbitrariness for the law.
Over time, through the development of follow-on work (Chapter~\ref{chapter:fairness}, Cooper et al.~\cite{cooper2024variance}), we have come to believe that this relationship is more significant than suggested in this chapter.
In particular, there remains important legal-theory work to more fully address the arbitrariness induced by stochasticity. 
We have begun follow-on work in this area, which we hope to complete later this year. 


==> section/30-algorithms/31-tunamh/999-tunamh-coda.tex <==
\section{Coda} \label{sec:tunamh:coda}

\todo{really beautiful modular code...and then it is not faster}
\todo{It's an empirical issue that the batch size changes every iter}


==> section/30-algorithms/33-tradeoffs/999-tradeoffs-coda.tex <==
\section{Coda}\label{sec:eaamo:coda}

\todo{Talk about how well this has aged; bigger and bigger models, trade-offs in modern distributed ML systems -- does not need to be a car, can be ChatGPT, MoE}

\todo{audits, security audits}

==> section/40-genai/43-talkinshort/9999-talkinshort-coda.tex <==
\section{Coda}\label{sec:talkinshort:coda}

\todo{reference to longer version; only become more significant; references to models piece; influence in scholarship, also law and policy; also a piece of work that has had influence in new field formation; workshop info; working on this a moving target}

==> section/references.tex <==
\iffalse
\bibliography{
references/references-1, 
references/references-a, 
references/references-b, 
references/references-c, 
references/references-d, 
references/references-e, 
references/references-f, 
references/references-g, 
references/references-h,
references/references-i, 
references/references-j,
references/references-k,
references/references-l,
references/references-m,
references/references-n,
references/references-o,
references/references-p,
references/references-q-r, 
references/references-s,
references/references-t-v,
references/references-w-z
}
\fi
